Sampling-based Exploration for Reinforcement Learning of Dexterous Manipulation

In this paper, we present a novel method for achieving dexterous manipulation of complex objects, while simultaneously securing the object without the use of passive support surfaces. We posit that a key difficulty for training such policies in a Reinforcement Learning framework is the difficulty of exploring the problem state space, as the accessible regions of this space form a complex structure along manifolds of a high-dimensional space. To address this challenge, we use two versions of the non-holonomic Rapidly-Exploring Random Trees algorithm; one version is more general, but requires explicit use of the environment's transition function, while the second version uses manipulation-specific kinematic constraints to attain better sample efficiency. In both cases, we use states found via sampling-based exploration to generate reset distributions that enable training control policies under full dynamic constraints via model-free Reinforcement Learning. We show that these policies are effective at manipulation problems of higher difficulty than previously shown, and also transfer effectively to real robots. Videos of the real-hand demonstrations can be found on the project website: https://sbrl.cs.columbia.edu/

==> litreview.tex <==
\hline

\section{Literature Review (To Be Deleted)}
\begin{enumerate}
    \item Human demonstrations for exploration
    \begin{enumerate}
        \item Dexterous manipulation with RL and Human Demonstrations \cite{Rajeswaran2017-au} 
        \item \cite{Radosavovic2021-pg} develop a method for using state only demonstrations for imitiation learning
        \item \cite{Abbeel2004-tu} apparenticeship learning via Inverse Reinforcement Learning
    \end{enumerate}
    \item Engineering reset state distributions
    \begin{itemize}
        \item \citeauthor{Nair2017-nu} use human demonstrations states as reset distribution for unstable tasks. They also observed that the behavior cloning was helpful in only a few instances.
        \item Ecoffet et al \cite{Ecoffet2019-lk, Ecoffet2021-xs} demonstrated that restarting exploration from previously visited states has significantly effective for classic hard-exploration problems in Atari domains and also for robot motion planning.
        \item \citeauthor{Tavakoli2018-ah} propose starting from an initial state and add explored states to a replay to restart exploration from for future rollouts and show improved performance for classic motor control tasks.
    \end{itemize}
    \item Combinining reinforcement learning with sample-based planning
    \begin{enumerate}
        \item A recent survey \cite{McMahon2022-nt} of the use of learning with sampling-based methods shows that this an active area of research with many interesting developments in recent years. The methods broadly aim to improve local planning in SBP with reinforcement learning agents and make useful predictors with supervised learning.
        \item \citeauthor{Francis2020-qe} train reinforcement learning agents to achieve short-range navigation and uses PRMs to map reachable goal space (PRM-RL).
        \item \citeauthor{Chiang2019-vm} learn local policy using reinforcement and bias RRT is directions deemed promising by learned reachability estimator to grow tree efficiently.
        \item \citeauthor{Schramm2022-hs} use RL policy to guide SST the state-of-the-art sampling-based method for motion planning 
        and show improved performance.
        \item Critical PRM \cite{Ichter2019-oi} learn to predict if a sampled node is critical and use it towards building a more efficient PRMs. This work also uses RL local policy.
        \item \citeauthor{Jurgenson2019-ye} use RRT* trajetories as expert demonstrations in DDDP-MP for robot arm motion planning.
        \item \citeauthor{Ha2020-od} use BiRRT trajectories as expert demonstrations for multi-arm motion planning. 
        \item \citeauthor{Morere2020-gq} also use expert demonstrations from RRT to initialize a policy.  
    \end{enumerate}
    \item{Sample-based planning}
        \begin{enumerate}
            \item RRT \citeauthor{LaValle1998-kn}
            \item \citeauthor{Kingston2018-wg} provide a survey of motion planning method with constraints
            \item \citeauthor{LaValle1999-zm} Randomized kinodynamic planning
            \item \citeauthor{Karaman2010-dw} \cite{Karaman2010-zi} RRT*
            \item \cite{Webb2013-nt} Kinodynamic RRT*
            \item \cite{Sucan2012-wm} KPIECE (algorithm for kinodynamic planning)
            \item PRM 
            \end{enumerate}
     \item Sampling-based planning for in-hand manipulation
     \begin{enumerate}
         \item \citeauthor{Leveroni1996-iy} build a grasp map and plan an grasp gait through search. 
         \item \citeauthor{Han1998-xj} rolling, sphere, non-holonomic motion planning
         \item \citeauthor{Yashima2003-lw} adapt RRT for in-hand manipulation while also selecting different contact modes in which to grow the tree.
         \item \citeauthor{Xu2007-yb} also use RRT for in-hand manipulation of a sphere.
     \end{enumerate}
     \item Miscellaneous
     \begin{enumerate}
         \item \citeauthor{Agarwal2020-zu} show theoretical results of improved sample efficiency of designing reset state distributions in policy gradient methods. a favorable initial state distribution provides a means to circumvent worst-case exploration issues.
         \item Pathak et al. \cite{Pathak2019-hp, Pathak2017-ik} curiosity driven exploration
         \item Parameter space noise \citeauthor{Plappert2017-ba} compute policy gradients when using parameter space.
         \item \citeauthor{Kohl2004-zs} first work to explore parameter space nosie.
         \item \citeauthor{Sehnke2010-nv} 
     \end{enumerate}
\end{enumerate}
\subsection{NOTES}
\begin{itemize}
    \item  Stable Sparse-RRT (SST) and it's optimal variant SST* \cite{Li2021-lv} are the state-of-the-art sampling-based methods for high-dimensional motion planning with physics.
    \item SoRB \cite{Eysenbach2019-rm} uses a buffer of states and connects them to form a graph for planning.
    \item Our work is conceptually most similar to LeaPER \cite{Pinto2018-xi} which also uses plans obtained by RRT as reset state distribution. LeaPER generates RRT with modified or quasi-static physics to generate plans which typically require domain knowledge. for simple non-prehensile manipulation tasks. While we also show the feasibility of quasistatic RRT to generate reset state distribution, we critically differ from LeaPER by demonstrating the feasibility of general non-holonomic RRT with complex dynamics.
    \item This approach assumes the feasibility of learning a local planner to transition between nearby states in the desired state-space. These approaches have been developed for navigation tasks where it is relatively straightforward to know the desired state-space. Attempting to follow this approach for dexterous manipulation directly leads us into a chicken or egg situation. In dexterous manipulation, the state-space is unintuitive. Training the local policy to reach nearby states requires concrete knowledge of the desired state-state space which is what we are after in the first place. Dexterous manipulation learning the local policy is itself hard and exploring the relevant states is even more difficult.
    \item PRMs are not suitable for our problem. For in-hand manipulation sampling a random point cannot provide reasonable coverage. We have to sample a point in a high dimensional non-convex space, next we have to check if it satisfies additional task independent and task specific constraints. 
    \item We cannot use RRT actions as expert demonstrations. They are far too few and are of not good quality to imitate. We cannot use them in the replay buffer either. Don't know what to do here.
    \item Exploration can be hard for too reasons. Typically, when people talk about hard exploration problems they mean problems with a large state space but its complex structure makes it results in sparse rewards. The dynamics is assumed to be non-deterring. A problem can also be hard to due to complex dynamics for example maintaining stability. In-hand manipulation checks both these boxes.
\end{itemize}




GPU based physics parallelism   While we show that quasi-static with projection ba

What kind or related work? We should look at work that use RRT with RL is some form.
We are ultimately using offline trajectories. This implies we should also talk about offline reinforcement learning methods and reinforcement learning with demonstrations. When we talk about RRT methods we should also mention paper related to projection method and also generic non-holonomic RRT

Thus there are the following categories:
1. Other RRT + RL
2. Offline RL
3. State-only demonstration

Offline reinforcement learning requires that the trajectories be valid. Ours are slow steps so they won't work. 


